Koopman-based Control of a Soft Continuum Manipulator Under Variable Loading Conditions

Controlling soft continuum manipulator arms is difficult due to their infinite degrees of freedom, nonlinear material properties, and large deflections under loading. This paper presents a data-driven approach to identifying soft manipulator models that enables consistent control under variable loading conditions. This is achieved by incorporating loads into a linear Koopman operator model as states and estimating their values online via an observer within the control loop. Using this approach, real-time, fully autonomous control of a pneumatically actuated soft continuum manipulator is achieved. In several trajectory following experiments, this controller is shown to be more accurate and precise than controllers based on models that are unable to explicitly account for loading. The manipulator also successfully performs pick and place of objects with unknown mass, demonstrating the efficacy of this approach in executing real-world manipulation tasks.

==> sections/02d_svd.tex <==
\subsection{Practical Considerations: Selection of Basis Functions and Dimensional Reduction}
\label{sec:svd}

The effectiveness of a finite-dimensional approximation $\bar{\koop}_{T_s}$ in representing the actions of the infinite-dimensional Koopman operator $\koop_{T_s}$ depends greatly upon the subspace upon which it is projected $\bar{\mathcal{F}}$, i.e. the span of the basis functions selected.

\Dan{finish rest of paper before coming back to complete this section. Only include if there is space.}


==> unused/01_intro_old.tex <==
\section{Introduction}  \label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/overview.pdf}
    \caption{Control of a pneumatic soft robot arm that is robust to changes to the load at the end effector is achieved using model predictive control and observer that provides online estimate the load. \Dan{Placeholder image. Elaborate once the figure is complete}}
    \label{fig:overview}
\end{figure}


Soft continuum manipulator arms are an active area of research in the robotics community.
They are lightweight, cheap to make, and their inherent compliance carries the promise to enable safe interaction with humans, delicate objects, and the environment ~\cite{immega1995ksi,hannan2001elephant,mcmahan2005design,grissom2006design,cianchetti2013stiff,mahl2014variable,hughes2016soft,phillips2018dexterous}.
These properties would make them ideal platforms for tasks involving physical human-robot interaction such as feeding~\cite{miller1998assistive} or sorting products in a warehouse~\cite{correll2016analysis}, yet the real-world application of soft manipulators has, so far, been limited.
This may be due to the difficulty of obtaining control-oriented models for systems that exhibit infinite degrees-of-freedom, nonlinear material properties, and unconventional actuation schemes \cite{george2018control}.
% Models are particularly hard to obtain for variable loading conditions that induce large deformations of the soft structure.
The lack of suitable models limits automatic control and it is not surprising that many (or: the most) successful soft robots to date are controlled via teleoperation to perform tasks such as object manipulation \cite{webster2010design} \Dan{Move this thing about teleoperation to later, and need better citation}.
% In practice, therefore, most soft manipulators must still be controlled via teleoperation (teleoperated) to perform tasks such as object manipulation \cite{webster2010design}.
\David{Can we restate the last sentence to say "The lack of suitable models limits automatic control and it is not surprising that many (or: the most) successful soft robots to date are controlled via teleoperation to perform tasks such as object manipulation \cite{webster2010design}.}

% %% Why soft manipulators are so difficult to model and control
% The challenge in modeling and controlling soft continuum manipulators stems from the fact that they exhibit distributed deformation throughout their bodies and thus an have infinite number of degrees of freedom.
% This limits the applicability of rigid-body methods for modeling and control, which rely on the assumption of a finite set of rigid links connected by discrete joints.
% Without the assumption of rigid links, nonlinear material properties must also be taken into account, further complicating the task of identifying a suitably accurate model for the purpose of automatic control.
% \David{"The primary challenge in modeling and controlling soft continuum manipulators, especially under load, is that their continuous deformation cannot be described by a finite set of degrees of freedom.
% This lack of discrete joints strongly limits the applicability of established rigid-body methods for modeling and control, which can only be used in combination with strongly simplifying assumptions about shape and deformation of the soft robot. In addition, the continuous deformation is subject to nonlinear material properties, even further complicating the task of identifying a suitably accurate model."}

% \David{It feels as in your head you are actually thinking about two different types of models.  One for feedforward control and one for feedback control.  You seem to assume that the feedforward model needs to be more precise.  It needs to be able to accurately predict deformations under load and let you figure out how to compensate for these deformation by applying the correct and exact pressure values to each free.  If your model is off, your resulting motion is completely off.  In the next paragraph, you seem to imply that the model for feedback can be simpler.  That's true, since in a sense it only needs to be representing a sense of direction and not one of scale. i.e., `if you want to go in this direction try putting pressure in these Frees.  Keep playing with the pressure value until you are there.'.  If you are thinking this way, try to express this idea more explicitely.}

%% Feedback is usually used to compensate for model uncertainty, but not good for soft robots
In manipulation, accurate models are particularly important for feedforward-control, where they are used to compensate for the effects of gravity and inertia.
Accurate feedforward models also allow for a reduction of the feedback gains and thus for an overall more compliant behavior.  When such accurate models are not available, feedback control can be used to some degree to offset the effects of model uncertainty and disturbances.
However, relying too heavily on feedback has been shown to reduce the compliance of soft robotic systems \cite{della2017controlling}.
That is, high-gain feedback might negate the desirable compliance of a soft robot by replacing its natural dynamics with those of a slower, stiffer system.

%% Justification for data-driven modeling
Recently, data-driven modeling techniques have emerged as a powerful tool for obtaining the accurate models required for feedforward control of soft continuum manipulators.
A primary benefit of these techniques is their ability to describe an input/output relationship from system observations. 
% without an explicit definition of the state.
% For soft robots, which exhibit virtually infinite degree-of-freedom motion, we are usually interested in
% The complete state of a soft continuum manipulator is infinite-dimensional
\David{You need to elaborate on the previous sentence. Why is this a benefit? Going back to the question of dimensionality, it allows you to do dimensionality reduction in a space that is potentially more meaningful than the shape of the robot.}
The input/output data that is necessary to create such models can be easily collected for soft robots.
Compared to conventional rigid-bodied manipulators, soft manipulators pose much less of a physical threat to themselves and their surroundings.
It is hence possible to automatically and safely collect data under a wide range of control inputs and operating conditions.

% Description of some previous work, and some downsides or caveats (i.e. localized deformations at soft joints)
% Make the case that other papers acheive control in a way that is not great because they don't produce nice control oriented models
% Mention Koopman here (maybe) along with some of it's benefits.
Within the class of data-driven methods, deep learning of artificial neural networks has been a popular approach to capture the nonlinear input/output behavior of soft robots.
For instance, \citet{thuruthel2018model} describe a recurrent neural network model for a pneumatically driven soft manipulator that was trained from data. 
To perform subsequent control, a closed-loop optimal control policy was generated using supervised reinforcement learning.
The resulting control policy enabled the manipulator to reach desired points in a two-dimensional workspace.
\citet{hyatt2019model} constructed a neural network model for a bellows-actuated manipulator from data, and three-dimensional position control was achieved using a model predictive controller.
Notably, the controller was based on a linearization of the full neural network model, since computing inputs in real-time using the full model was computationally infeasible.  
Theses examples illustrate two fundamental downsides of using neural network models for control. 
First, building a neural network model requires solving a nonlinear optimization problem for which global convergence may not be guaranteed and second, utilizing this model at run-time is non-trivial since the control input usually appear non-linearly within the computed model. 
\Dan{Also need to cite Girish Chowdhary paper \cite{satheeshbabu2019open}, which used deep reinforcement learning for open loop position control of soft arm. ALso Andrew Marchese paper using iterative learning control \cite{marchese2014autonomous}}
\Ram{may also want to mention that these models have not been applied to pick and place with soft robots...}
% making them incompatible with realtime control in most cases.

%% Indroducing Koopman! and Why Koopman is great
In contrast to deep learning methods, Koopman operator theory offers a data-driven modeling approach that yields explicit, control-oriented models by identifying a linear embedding of system dynamics in an infinite-dimensional function space \cite{budivsic2012applied}\cite[Ch. 7]{brunton2019data}.
The approach leverages the linear structure of the Koopman operator to construct linear models of nonlinear controlled dynamical systems from input/output data \cite{bruder2019nonlinear, mauroy2016linear}, and to control them using established linear control methods.
In theory, this approach involves \emph{lifting} into an infinite-dimensional space of scalar functions (referred to as observables), where the flow of such functions along trajectories of the nonlinear dynamical system is described by the \emph{linear} Koopman operator.
In practice, however, it is infeasible to compute an infinite-dimensional operator, so a process called Extended Dynamic Mode Decomposition (EDMD) \cite{williams2015data} is typically employed to compute a finite-dimensional projection of the Koopman operator onto a finite-dimensional subspace of all observables (scalar functions).
% This approximation of the Koopman operator describes the evolution of the output variables themselves, provided that they lie within the finite subspace of observables upon which the operator is projected.
Hence, this approach makes it possible to control the output of a nonlinear dynamical system using a controller designed for its linear Koopman representation \cite{Abraham-RSS-17, korda2018linear}.
\Ram{technically our approach and T. Murphey's approach are a bit different...}
% \Dan{I think this paragraph can be shortened}

% Examples of successful Koopman control
A Koopman-based approach has been successfully used to control several rigid-bodied robots such as a Sphero SPRK,  \cite{Abraham-RSS-17}, a quadcopter \cite{abraham2019active}, a robotic fish \cite{mamakoukas2019local}, and the 2D configuration of the end effector of a soft robot arm \cite{Vasudevan-RSS-19}.
Despite their ability to construct models that are amenable to online control, these Koopman-based methods have not yet been applied to perform control of soft robot manipulators during tasks that involve variable loading conditions, such as
pick and place. 
% This is because the effect of loading can vary during a pick and place task.
For such tasks, the effect of loading on the model must somehow be estimated and updated during real-time operation.
\David{The addition of loading in this paragraph seems to be a bit of an afterthought.  Given that the primary innovation from your side is to work on loads, I would try to include the notion and effect of load more prominently in the introduction.  I tried to mentioned it more in my edits, but maybe you can state it in a more fundamental manner:  What changes when you have to think about loads?}

% Despite their ability to construct models that are amenable to performing online control, these Koopman-based models are unable to account for disturbances that do not appear consistently throughout the model identification process.
% For example, consider the case of identifying a model of a manipulator with variable loading at its end-effeector using Koopman

% in the case of identifying a model of a manipulator that may encounter variable loading. 



% However, Koopman-based models do still suffer from one of the fundamental shortcomings of data-driven models, which is the inability to accurately predict/describe system behavior under conditions not present/accounted for in their training data set.
% % Control accuracy can be maintained in the presence of unmodeled conditions using feedback control, but as previously stated too much feedback effectively reduces the compliance of soft manipulators, negating their unique characteristics.
% Thus, it is important to explicitly account for any variable conditions that the system is likely to encounter during regular operation and include examples of those conditions in the training set.

% In the case of manipulators, control performance should be invariant to the payload at the end effector.
% This not only requires that the payload be explicitly incorporated into any data-driven model, but also that the it be measured or estimated during realtime operation.
% \Dan{This paragraph needs help.}

%% In this work, we present a data-driven modeling and control approach for soft robots that incorporates loads
\Ram{list out contributions...}
This work presents a method for incorporating loading conditions into a Koopman-based modeling and control framework and demonstrates real-time, fully autonomous control of a pneumatically actuated soft continuum manipulator with variable payload.
This approach yields a more consistent control performance over a variety of loading conditions than several comparison model-based controllers.
To the best of the authors' knowledge, this is the first implementation of a closed-loop controller for a soft continuum manipulator that explicitly accounts for loading, and the first successful pick and place demonstration by a soft continuum manipulator. \David{If this is true, you need to play that card much sooner in your intro and highlight the challenges of adding load.}

%% Outline
The rest of this paper is organized as follows:
Section \ref{sec:sysid} formally introduces the Koopman operator and describes how to construct models of nonlinear dynamical systems from data. 
Section \ref{sec:loadest} introduces a method for incorporating loading conditions into the model. 
Section \ref{sec:mpc} describes our Koopman-based model predictive controller and a method for estimating loading conditions online.
Section \ref{sec:experiments} describes the set of experiments used to evaluate the performance of our Koopman-based model predictive controller on a pneumatically actuated soft continuum manipulator, including trajectory following while carrying an unknown payload, and autonomously sorting objects by mass.
Section \ref{sec:discussion} discusses the results of these experiments and concludes the paper. 






%% UNUSED/OLD TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %% Why soft manipulators are not capable of doing things, using examples
% Robotic manipulator arms meant to assist humans with \Dan{collaborative} tasks such as feeding \cite{miller1998assistive} or sorting objects into boxes \cite{correll2016analysis} could also benefit from the inherent safety and adaptability of soft materials.
% However, the dynamics of soft manipulators can be difficult to model and control due to the high number of degrees of freedom present and the non-linear material properties they exhibit \Dan{look to prev better for better working of this sentence}.
% Typical rigid-body methods for modeling which assume rigid links between components can not longer be used.
% Because of this, soft manipulator arms are not yet capable of autonomously performing basic assistive tasks such as object manipulation \cite{hughes2016soft}\Dan{verify this source backs-up this claim}.

% This is espeically notable for many soft robots, whose body mass/inertia is much smaller tha

% In \cite{Vasudevan-RSS-19} Koopman operator theory was used to construct a high-dimensional linear model of pneumatic soft robot arm actuated by McKibben artifical muscles \cite{tondu2012modelling} and achieve accurate trajectory following using model predictive control. 

% %% Summary of Contributions
% The theoretical contributions of this work are \Dan{@Ram I'm interested on your input here...}:
% \begin{itemize}
%     \item Method for incorporating external loading into data-driven Koopman models
%     \item Optional: Method for dimensional reduction of Koopman models \Dan{Not really novel, just possibly in the Koopman context}
% \end{itemize}
% The practical contributions of this work are:
% \begin{itemize}
%     \item Achieved (autonomous) control of a (completely) soft robot arm.
%     \item Demonstrated control performance that is robust to changes in external loading conditions. \Dan{but note that they have to be modeled loading conditions, this is not robustness to unmodelled disturbances.}
%     \item Demonstrated that (autonomous) object manipulation/sorting is possible with (completely) soft manipulator.
%     \item To the best of the authors knowledge, no soft manipulator has yet been shown executing a pick-and-place task autonomously (using closed-loop automatic control).
% \end{itemize}

% % Description of previous work
% Data-driven approaches have been successfully utilized in 
% Data-driven models have already been used to successfully to control several soft robots.
% In \cite{gillespie2018learning} and \cite{thuruthel2018model} neural network models trained from experimental data were identified, then used in a model-based control framework to achieve accurate \Dan{position} control of a soft arm.
% In \Dan{Koopman stuff?}
% Using neural network models trained from experimental data, accurate \Dan{position} control of a soft robot arm was achieved in \cite{gillespie2018learning} and \cite{thuruthel2018model}.
% Neural net plus linearization or something \cite{hyatt2019model} \Dan{This one is continuum}.
% Control of soft arm with unknown load, but robot has joints \cite{terry2019adaptive} \Dan{This has pneumatic joints}.

% \Dan{This paper is about cosserot model with loading of the Octarm \cite{trivedi2008geometrically}}
% \Dan{A similar approach was used to control a pneumatic soft manipulator with unknown payloads with psudo-joints \cite{terry2019adaptive}, but to the best the authors' knowledge, this is the first implementation of such control using a continuum style soft manipulator.}

% % High level introduction
% \Dan{THIS JUST HERE FOR MY REFERENCE, IT'S THE SPARKNOTES VERSION OF THE INTRO:
% Soft robots are desirable for tasks that include close interaction with humans and the environment due to the inherent safety, resilience, and --- associated with soft structures.
% For this reason (due to these benefits/characteristics), soft robots have been developed to... (wearable orthotics, biomimicry swimming and snakes.
% However, soft robots are not yet capable of performing basic assistive tasks such as object manipulation.
% Recent research has shown that control of soft robots is achievable by identifying a linear embedding of their dynamics from data, then employing linear model-based control techniques \cite{bruder2019nonlinear, Vasudevan-RSS-19} (CITE TRO?).
% In this paper, we utilize such an approach to develop a framework by which a soft robot arm is capable of performing pick-and-place of objects of unknown mass.
% }

==> unused/intro_rough.tex <==

\Dan{Pick-and-place is a common task in places like Amazon packaging facilities, but is typically done by humans because they need to be able to grasp objects of a bunch of different shapes, sizes, masses, and most industrial robots aren't effective under such variable/unknown conditions.}
Automation plays a key role in modern packaging facilities, such as those of Amazon (CITE AMAZON PACKAGING CENTER DESCRIPTION), where ---- robots are used to efficiently move goods within a warehouse.
However, the task of picking objects from large pallets/shelves and placing them in designated containers is still almost exclusively performed by humans. 
This task, deemed ``pick-and-place'' requires object recognition, pose recognition, grasp planning, compliant manipulation, motion planning, task planning, task execution, and error detection and recovery, making commercially viable automated ``pick-and-place'' in unstructured environments a difficult/lingering challenge (CITE AMAZON PICKING CHALLENGE RULES).
(Is this too specific? Maybe the motivation should be broader in scope?)

\Dan{Soft grippers have enabled some automation of this type of task, because they passively adapt to shapes.}
While many of th

\Dan{BUT, they are attached to rigid robots which still pose a serious safety threat to human operators.}

\Dan{Soft robot arms can solve this problem because they have inherent safety for tasks that involve human collaboration/proximity.}

\Dan{Challenge is in controlling them, because they have weird dynamics, blah blah blah...}

\Dan{Recent work has shown that control is possible using Koopman (self cite)}

\Dan{In this work we expand on that approach to incorporate loads, and demonstrate the approach by performing pick-and-place with a soft robot arm.}

\Dan{Potential angle (but perhaps to big of a generalization):
For large rigid bodied robots, the mass of objects is negligible with respect to the arm. Therefore control can be reduced to a kinematics problem. For pneumatically driven soft robot arms this is not the case, sense the mass of the arm is low by comparison.
}

==> unused/intro_rough_2.tex <==
\section{Introduction}  \label{sec:intro}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/overview.pdf}
    \caption{Control of a pneumatic soft robot arm that is robust to changes to the load at the end effector is achieved using model predictive control and observer that provides online estimate the load. \Dan{Placeholder image. Elaborate once the figure is complete}}
    \label{fig:overview}
\end{figure}


Soft continuum manipulator arms are an active area of research in the robotics community.
They are lightweight, cheap to make, and their inherent compliance carries the promise to enable safe interaction with humans, delicate objects, and the environment ~\cite{immega1995ksi,hannan2001elephant,mcmahan2005design,grissom2006design,cianchetti2013stiff,mahl2014variable,hughes2016soft,phillips2018dexterous}.
These properties would make them ideal platforms for tasks involving physical human-robot interaction such as feeding~\cite{miller1998assistive} or sorting products in a warehouse~\cite{correll2016analysis}, yet the real-world application of soft manipulators has, so far, been limited.
This may be due to the difficulty of obtaining control-oriented models for systems that exhibit infinite degrees-of-freedom, nonlinear material properties, and unconventional actuation schemes \cite{george2018control}.
% Models are particularly hard to obtain for variable loading conditions that induce large deformations of the soft structure.
The lack of suitable models limits automatic control and it is not surprising that many (or: the most) successful soft robots to date are controlled via teleoperation to perform tasks such as object manipulation \cite{webster2010design} \Dan{Move this thing about teleoperation to later, and need better citation}.
\David{Can we restate the last sentence to say "The lack of suitable models limits automatic control and it is not surprising that many (or: the most) successful soft robots to date are controlled via teleoperation to perform tasks such as object manipulation \cite{webster2010design}.}

% Soft robots are able to safely interact with humans and delicate objects by deforming continuously to passively adapt their shape to their surroundings,
% This has made soft robots attractive for a wide array of potential applications \cite{ilievski2011soft,marchese2014autonomous,tolley2014resilient,zhao2016helping,sinatra2019ultragentle,coad2019vine,moore-danforth}. 

% Many novel soft robots have been developed that leverage these unique characteristics to achieve safe human-robot interaction  \cite{ilievski2011soft,zhao2016helping,sinatra2019ultragentle}, exploration of unstructured environments \cite{tolley2014resilient,coad2019vine}, or even mimicry of biological systems \cite{marchese2014autonomous,moore-danforth}.
% Soft robotic manipulator arms~\cite{immega1995ksi,hannan2001elephant,mcmahan2005design,grissom2006design,cianchetti2013stiff,mahl2014variable,hughes2016soft,phillips2018dexterous} are a particularly important application of soft robotics since these arms are inherently compliant and can safely interact with delicate objects and the environment.

% Examples include soft orthotic devices \cite{zhao2016helping}, grippers \cite{ilievski2011soft,sinatra2019ultragentle}, growing ``vine'' robots \cite{coad2019vine}, crawlers \cite{tolley2014resilient}, and biomimetic robots that emulate fish \cite{marchese2014autonomous} and snakes \cite{moore-danforth}, just to name a few.
% \Dan{I think I should delete this first paragraph}.

%% Shortcoming of current soft manipulators
% Several soft robotic manipulator arms have also been developed such as Octarm \cite{grissom2006design}, Wood arm \cite{phillips2018dexterous}, STIFF-FLOP \cite{cianchetti2013stiff}, Air-Octor \cite{mcmahan2005design}, Elephant trunk robot \cite{hannan2001elephant},  KSI tentacle manipulator \cite{immega1995ksi}, Festo Bionic Handling Assistant \cite{mahl2014variable}, among others \cite{hughes2016soft} \Dan{clean up this sentence}.
% These arms can exploit their inherent compliance to safely interact with delicate objects and the environment.
% This should make them well suited for automating tasks that involve physical human-robot interaction such as feeding \cite{miller1998assistive}, or sorting objects in a warehouse \cite{correll2016analysis}, \Dan{Add third task here}.
% However, autonomous execution of these types of tasks remains an open challenge due to the difficulty involved in modeling and controlling soft robots, especially under variable loading conditions.
% In practice, therefore, most soft manipulators must still be controlled via teleoperation (teleoperated) to perform tasks such as object manipulation \cite{webster2010design}.

%% Why soft manipulators are so difficult to model and control
The challenge in modeling and controlling soft continuum manipulators stems from the fact that they exhibit distributed deformation throughout their bodies and thus an have infinite number of degrees of freedom.
This limits the applicability of rigid-body methods for modeling and control, which rely on the assumption of a finite set of rigid links connected by discrete joints.
Without the assumption of rigid links, nonlinear material properties must also be taken into account, further complicating the task of identifying a suitably accurate model for the purpose of automatic control.
\David{"The primary challenge in modeling and controlling soft continuum manipulators, especially under load, is that their continuous deformation cannot be described by a finite set of degrees of freedom.
This lack of discrete joints strongly limits the applicability of established rigid-body methods for modeling and control, which can only be used in combination with strongly simplifying assumptions about shape and deformation of the soft robot. In addition, the continuous deformation is subject to nonlinear material properties, even further complicating the task of identifying a suitably accurate model."}

\David{It feels as in your head you are actually thinking about two different types of models.  One for feedforward control and one for feedback control.  You seem to assume that the feedforward model needs to be more precise.  It needs to be able to accurately predict deformations under load and let you figure out how to compensate for these deformation by applying the correct and exact pressure values to each free.  If your model is off, your resulting motion is completely off.  In the next paragraph, you seem to imply that the model for feedback can be simpler.  That's true, since in a sense it only needs to be representing a sense of direction and not one of scale. i.e., `if you want to go in this direction try putting pressure in these Frees.  Keep playing with the pressure value until you are there.'.  If you are thinking this way, try to express this idea more explicitely.}

%% Feedback is usually used to compensate for model uncertainty, but not here

In cases where an accurate model is unavailable, feedback control is typically used to offset the effects of model uncertainty and disturbances.
However, relying too heavily on feedback to compensate for model inaccuracy has been illustrated to reduce the compliance of soft robotic systems \cite{della2017controlling}.
That is, excessive feedback negates the desirable compliance of a soft robot by replacing its natural dynamics with those of a slower, stiffer system.
To limit the dependence on feedback and preserve compliance of soft robots while achieving adequate control performance, sufficiently accurate models are needed.
% \Dan{I can probably delete this paragraph now too... I think it was important for an earlier version}
\David{In manipulation, accurate models are particularly important for feedforward-control, where they are used to compensate for the effects of gravity and inertia.  Acurate feedforward models also allow for a reduction of the feedback gains and thus for an overall more compliant behavior.  When such accurate models are not available, feedback control can be used to some degree to offset the effects of model uncertainty and disturbances. However, relying too heavily on feedback has been shown to reduce the compliance of soft robotic systems \cite{della2017controlling}. That is, high-gain feedback might negate the desirable compliance of a soft robot by replacing its natural dynamics with those of a slower, stiffer system.}

%% Justification for data-driven modeling
\David{To obtain the acurate models required for feed forward control, ...}Recently, data-driven modeling techniques have emerged as a powerful tool for representing the input/output behavior of soft manipulators.
A primary benefit of these techniques is their ability to describe an input/output relationship from system observations. \David{You need to elaborate on the previous sentence. Why is this a benefit? Going back to the question of dimensionality, it allows you to do dimensionality reduction in a space that is potentially more meaningful than the shape of the robot.}
These data-driven methods are especially well suited for soft manipulators since soft robots pose less of a physical threat to themselves and their surroundings when subjected to arbitrary control inputs when compared to conventional rigid-bodied manipulators. 
This property of soft robotic systems makes it possible to safely collect input/output data over a wide range of operating conditions in an automated fashion.
\David{"The input-output data that is necessary to create such models can be easily collected for soft robots. Compared to conventional rigid-bodied manipulators, they pose much less of a physical threat to themselves and their surroundings. It is hence possible to subject them to arbitrary control inputs and thus automatically and safely collect input/output data over a wide range of operating conditions."}

% Description of some previous work, and some downsides or caveats (i.e. localized deformations at soft joints)
% Make the case that other papers acheive control in a way that is not great because they don't produce nice control oriented models
% Mention Koopman here (maybe) along with some of it's benefits.
\David{Within the class of data-driven models, } Deep learning of artificial neural networks has been a popular data-driven \David{remove data-driven if you use the opening part} approach to capture the nonlinear input/output behavior of soft robots.
For instance, \citet{thuruthel2018model} describe a recurrent neural network model for a pneumatically driven soft manipulator that was trained from data. 
To perform subsequent control, a closed-loop optimal control policy was generated using supervised reinforcement learning.
The resulting control policy enabled the manipulator to reach desired points in a two-dimensional workspace.
\citet{hyatt2019model} constructed a neural network model for a bellows-actuated manipulator from data, and three-dimensional position control was achieved using a model predictive controller.
Notably, the controller was based on a linearization of the full neural network model, since computing inputs in real-time using the full model was computationally infeasible.  
This exemplifies/illustrates the two fundamental downsides of using neural network models for control. 
First, building a neural network model requires solving a nonlinear optimization problem for which global convergence may not be guaranteed and second, utilizing this model at run-time is non-trivial since the control input usually appear non-linearly within the computed model. 
\Dan{Also need to cite Girish Chowdhary paper \cite{satheeshbabu2019open}, which used deep reinforcement learning for open loop position control of soft arm. ALso Andrew Marchese paper using iterative learning control \cite{marchese2014autonomous}}
\Ram{may also want to mention that these models have not been applied to pick and place with soft robots...}
% making them incompatible with realtime control in most cases.

%% Indroducing Koopman! and Why Koopman is great
In contrast to deep learning methods, Koopman operator theory offers a data-driven modeling approach that yields explicit, control-oriented models by identifying a linear embedding of system dynamics in an infinite-dimensional function space \cite{budivsic2012applied}\cite[Ch. 7]{brunton2019data}.
The approach leverages the linear structure of the Koopman operator to construct linear models of nonlinear controlled dynamical systems from input/output data \cite{bruder2019nonlinear, mauroy2016linear}, and to control them using established linear control methods.
In theory, this approach involves \emph{lifting} into an infinite-dimensional space of scalar functions (referred to as observables), where the flow of such functions along trajectories of the nonlinear dynamical system is described by the \emph{linear} Koopman operator.
In practice, however, it is infeasible to compute an infinite-dimensional operator, so a process called Extended Dynamic Mode Decomposition (EDMD) \cite{williams2015data} is typically employed to compute a finite-dimensional projection of the Koopman operator onto a finite-dimensional subspace of all observables (scalar functions).
% This approximation of the Koopman operator describes the evolution of the output variables themselves, provided that they lie within the finite subspace of observables upon which the operator is projected.
Hence, this approach makes it possible to control the output of a nonlinear dynamical system using a controller designed for its linear Koopman representation \cite{Abraham-RSS-17, korda2018linear}.
\Ram{technically our approach and T. Murphey's approach are a bit different...}
% \Dan{I think this paragraph can be shortened}

% Examples of successful Koopman control
A Koopman-based approach has been successfully used to control several rigid-bodied robots such as a Sphero SPRK,  \cite{Abraham-RSS-17}, a quadcopter \cite{abraham2019active}, a robotic fish \cite{mamakoukas2019local}, and the 2D configuration of the end effector of a soft robot arm \cite{Vasudevan-RSS-19}.
Despite their ability to construct models that are amenable to online control, these Koopman-based methods have not yet been applied to perform control of soft robot manipulators during tasks that involve variable loading conditions, such as
pick and place. 
% This is because the effect of loading can vary during a pick and place task.
For such tasks, the effect of loading on the model must somehow be estimated and updated during real-time operation.
\David{The addition of loading in this paragraph seems to be a bit of an afterthought.  Given that the primary innovation from your side is to work on loads, I would try to include the notion and effect of load more prominently in the introduction.  I tried to mentioned it more in my edits, but maybe you can state it in a more fundamental manner:  What changes when you have to think about loads?}

% Despite their ability to construct models that are amenable to performing online control, these Koopman-based models are unable to account for disturbances that do not appear consistently throughout the model identification process.
% For example, consider the case of identifying a model of a manipulator with variable loading at its end-effeector using Koopman

% in the case of identifying a model of a manipulator that may encounter variable loading. 



% However, Koopman-based models do still suffer from one of the fundamental shortcomings of data-driven models, which is the inability to accurately predict/describe system behavior under conditions not present/accounted for in their training data set.
% % Control accuracy can be maintained in the presence of unmodeled conditions using feedback control, but as previously stated too much feedback effectively reduces the compliance of soft manipulators, negating their unique characteristics.
% Thus, it is important to explicitly account for any variable conditions that the system is likely to encounter during regular operation and include examples of those conditions in the training set.

% In the case of manipulators, control performance should be invariant to the payload at the end effector.
% This not only requires that the payload be explicitly incorporated into any data-driven model, but also that the it be measured or estimated during realtime operation.
% \Dan{This paragraph needs help.}

%% In this work, we present a data-driven modeling and control approach for soft robots that incorporates loads
\Ram{list out contributions...}
This work presents a method for incorporating loading conditions into a Koopman-based modeling and control framework and demonstrates real-time, fully autonomous control of a pneumatically actuated soft continuum manipulator with variable payload.
This approach yields a more consistent control performance over a variety of loading conditions than several comparison model-based controllers.
To the best of the authors' knowledge, this is the first implementation of a closed-loop controller for a soft continuum manipulator that explicitly accounts for loading, and the first successful pick and place demonstration by a soft continuum manipulator. \David{If this is true, you need to play that card much sooner in your intro and highlight the challenges of adding load.}

%% Outline
The rest of this paper is organized as follows:
Section \ref{sec:sysid} formally introduces the Koopman operator and describes how to construct models of nonlinear dynamical systems from data. 
Section \ref{sec:loadest} introduces a method for incorporating loading conditions into the model. 
Section \ref{sec:mpc} describes our Koopman-based model predictive controller and a method for estimating loading conditions online.
Section \ref{sec:experiments} describes the set of experiments used to evaluate the performance of our Koopman-based model predictive controller on a pneumatically actuated soft continuum manipulator, including trajectory following while carrying an unknown payload, and autonomously sorting objects by mass.
Section \ref{sec:discussion} discusses the results of these experiments and Section \ref{sec:conclusion} concludes the paper. 






%% UNUSED/OLD TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %% Why soft manipulators are not capable of doing things, using examples
% Robotic manipulator arms meant to assist humans with \Dan{collaborative} tasks such as feeding \cite{miller1998assistive} or sorting objects into boxes \cite{correll2016analysis} could also benefit from the inherent safety and adaptability of soft materials.
% However, the dynamics of soft manipulators can be difficult to model and control due to the high number of degrees of freedom present and the non-linear material properties they exhibit \Dan{look to prev better for better working of this sentence}.
% Typical rigid-body methods for modeling which assume rigid links between components can not longer be used.
% Because of this, soft manipulator arms are not yet capable of autonomously performing basic assistive tasks such as object manipulation \cite{hughes2016soft}\Dan{verify this source backs-up this claim}.

% This is espeically notable for many soft robots, whose body mass/inertia is much smaller tha

% In \cite{Vasudevan-RSS-19} Koopman operator theory was used to construct a high-dimensional linear model of pneumatic soft robot arm actuated by McKibben artifical muscles \cite{tondu2012modelling} and achieve accurate trajectory following using model predictive control. 

% %% Summary of Contributions
% The theoretical contributions of this work are \Dan{@Ram I'm interested on your input here...}:
% \begin{itemize}
%     \item Method for incorporating external loading into data-driven Koopman models
%     \item Optional: Method for dimensional reduction of Koopman models \Dan{Not really novel, just possibly in the Koopman context}
% \end{itemize}
% The practical contributions of this work are:
% \begin{itemize}
%     \item Achieved (autonomous) control of a (completely) soft robot arm.
%     \item Demonstrated control performance that is robust to changes in external loading conditions. \Dan{but note that they have to be modeled loading conditions, this is not robustness to unmodelled disturbances.}
%     \item Demonstrated that (autonomous) object manipulation/sorting is possible with (completely) soft manipulator.
%     \item To the best of the authors knowledge, no soft manipulator has yet been shown executing a pick-and-place task autonomously (using closed-loop automatic control).
% \end{itemize}

% % Description of previous work
% Data-driven approaches have been successfully utilized in 
% Data-driven models have already been used to successfully to control several soft robots.
% In \cite{gillespie2018learning} and \cite{thuruthel2018model} neural network models trained from experimental data were identified, then used in a model-based control framework to achieve accurate \Dan{position} control of a soft arm.
% In \Dan{Koopman stuff?}
% Using neural network models trained from experimental data, accurate \Dan{position} control of a soft robot arm was achieved in \cite{gillespie2018learning} and \cite{thuruthel2018model}.
% Neural net plus linearization or something \cite{hyatt2019model} \Dan{This one is continuum}.
% Control of soft arm with unknown load, but robot has joints \cite{terry2019adaptive} \Dan{This has pneumatic joints}.

% \Dan{This paper is about cosserot model with loading of the Octarm \cite{trivedi2008geometrically}}
% \Dan{A similar approach was used to control a pneumatic soft manipulator with unknown payloads with psudo-joints \cite{terry2019adaptive}, but to the best the authors' knowledge, this is the first implementation of such control using a continuum style soft manipulator.}

% % High level introduction
% \Dan{THIS JUST HERE FOR MY REFERENCE, IT'S THE SPARKNOTES VERSION OF THE INTRO:
% Soft robots are desirable for tasks that include close interaction with humans and the environment due to the inherent safety, resilience, and --- associated with soft structures.
% For this reason (due to these benefits/characteristics), soft robots have been developed to... (wearable orthotics, biomimicry swimming and snakes.
% However, soft robots are not yet capable of performing basic assistive tasks such as object manipulation.
% Recent research has shown that control of soft robots is achievable by identifying a linear embedding of their dynamics from data, then employing linear model-based control techniques \cite{bruder2019nonlinear, Vasudevan-RSS-19} (CITE TRO?).
% In this paper, we utilize such an approach to develop a framework by which a soft robot arm is capable of performing pick-and-place of objects of unknown mass.
% }

==> unused/outline.tex <==
\section{Outline}   \label{sec:outline}

\begin{outline}[enumerate]
    \1 Introduction
        \2 Pick-and-place is a common/useful task almost exclusively done by humans.
        \2 Soft grippers make grasping possible, but safety still a concern
        \2 Soft arm would be safe (and still accurate enough)
        \2 Recent work has shown this may be possible (self-cite)
        \2 Summary of contributions of this work.
    \1 Theory
        \2 Koopman system identification overview
        \2 Construction of load observer
        \2 Koopman MPC controller
    \1 Experiments
        \2 Description of robot
            \3 Composition of arm
            \3 Choice of gripper (can grasp a variety of objects without much control)
            \3 Regulators, cameras, etc.
        \2 Sysid
            \3 Gather data of robot arm with various known loads attached to end effector.
            \3 Fit Koopman model with the load as a state.
            \3 Build model and observer to estimate the load during operation.
        \2 Control
            \3 Pick and place objects with unknown mass (some in training data, some not). Measure deviation from desired placement point.
            \3 Throw objects of unknown mass into a bucket.
    \1 Conclusion
\end{outline}
